Enhancing Bug Reports for Mobile Apps

The modern software development landscape has seen a shift in focus toward mobile applications as "smart" devices near ubiquitous adoption. Due to this trend, the complexity of mobile applications has been increasing, making development and maintenance particularly challenging. However, it is clear that current bug tracking systems are not able effectively support construction of reports with actionable information that will directly lead to a bug's resolution. To address the need for an improved reporting system, we introduce a novel solution, called FUSION, that helps users auto-complete reproduction steps in bug reports for mobile apps. FUSION links information, that users provide, to program artifacts extracted through static and dynamic analysis performed before testing or release. The approach that FUSION employs is generalizable to other current mobile software platforms, and constitutes a new method by which off-device bug reporting can be conducted for mobile software projects. We evaluate FUSION by conducting a study that quantitatively and qualitatively measures the user experience of the system for both reporting and reproducing bugs, as well as the quality of the bug reports it produces. In a study involving 28 participants we apply FUSION to support the maintenance tasks of reporting and reproducing defects on 15 real-world bugs found in 14 open source Android apps. Our results demonstrate that FUSION allows for more reliable reproduction of bugs from reports by aiding users in reporting more detailed application-specific information compared to traditional bug tracking systems.

==> abstract.tex <==
\large
\noindent 
\begin{flushleft}
Software bug reports are artifacts leveraged by users, testers or developers in order to document defects in software applications or projects. Bug reports are typically instantiated when a problem (e.g. unexpected or unwanted behavior) is observed in a software application and are created through a mechanism known as an issue-tracker. The primary purpose of issue-tracking systems are to allow reporters to construct a detailed bug report that accurately describes a software problem so that it can be faithfully reproduced and subsequently fixed. In general, issue-trackers employ natural language descriptions of problems, and sometimes support the addition of augmented information such as the uploading of screenshots. These systems have been used, with few exceptions, mostly unchanged to document and formulate fixes for bugs across many different types of software projects. However, some applications that rely on complex user interactions are not well suited to these types of traditional systems, as they are not able to capture intricacies of complicated application event-flows. The most prominent example of a classification of applications that exhibits this type of behavior, and for which issue-tracking systems could be improved, is the rapidly growing category of mobile apps which rely on touch-based gestures for navigation on smartphones and tablet devices.
\end{flushleft}

\begin{flushleft}
 The modern software development landscape has seen a shift in focus toward mobile applications as ``smart" devices near ubiquitous adoption. Due to this trend, the complexity of mobile applications has been increasing, making development and maintenance particularly challenging. However, it is clear that current bug tracking systems are not able effectively support construction of reports with actionable information that will directly lead to a bug's resolution. To address the need for an improved reporting system, we introduce a novel solution, called FUSION, that helps users auto-complete reproduction steps in bug reports for mobile apps. FUSION links information, that users provide, to program artifacts extracted through static and dynamic analysis performed before testing or release. The approach that FUSION employs is generalizable to other current mobile software platforms, and constitutes a new method by which off-device bug reporting can be conducted for mobile software projects. We evaluate FUSION by conducting a study that quantitatively and qualitatively measures the user experience of the system for both reporting and reproducing bugs, as well as the quality of the bug reports it produces. In a study involving 28 participants we apply FUSION to support the maintenance tasks of reporting and reproducing defects on 15 real-world bugs found in 14 open source Android apps. Our results demonstrate that FUSION allows for more reliable reproduction of bugs from reports by aiding users in reporting more detailed application-specific information compared to traditional bug tracking systems.\\
\end{flushleft}



==> acknowledge.tex <==
\begin{flushleft}
\noindent This thesis and the work performed towards its writing would not have been possible without the support and guidance of several individuals.  First and foremost, I would like to thank my advisor, Dr. Denys Poshyvanyk for taking the time to mentor and support a physics major with an initially limited background in computer science.  He has tirelessly supported this work and set a great example illustrating how to conduct meaningful research in the field of software engineering with integrity, vision, passion and thoroughness.  It goes without saying that without him this work would not have been possible, and I look forward to continuing to grow as a researcher under his mentorship as I pursue my PhD.  \\
\end{flushleft}

\begin{flushleft}
\noindent Next, I would like to thank all of the members of the SEMERU group for their support in this project and others as I began my career as a graduate student.  It is not often that you find individuals who are willing to use their time to explain proper research methods and code conventions to a new research student and I am extremely grateful for their guidance.  In particular, I would thank to Mario Linares-V\'asquez, Carlos Bernal-C\'ardenas, and Christopher Vendome.  Mario, your research expertise and constructive feedback contributed immensely to this project and to my education as a software engineer and research practitioner.  Carlos, your coding expertise and patience in teaching me new techniques has been invaluable to me and this project.  Chris, I am grateful for your support and friendship  since I started at William \& Mary.  I cannot possibly give you all enough credit.\\
\end{flushleft}

\begin{flushleft}
\noindent I thank my parents Brian and Elizabeth for their continued support of my academic pursuits, especially during difficult times.  I look to you both for inspiration and motivation in the way you have raised my brothers and me and in the way you live your lives. I would also like to thank my grandparents, Tom and Jeanne Moran, and Mary and Paul Lavin, for always encouraging me in my studies and offering crucial advice when needed.\\
\end{flushleft}

\begin{flushleft}
\noindent Most Importantly, I would like to thank my fianc\'ee Emily for her unwavering support, especially during the late nights and deadline work marathons.  Your character and accomplishments inspire all that I do, and my full appreciation for having you in my life can not be adequately put into words.\\
\end{flushleft}


==> vita.tex <==
Kevin Moran has been working towards his Master's degree in computer science at the College of William & Mary since the Fall of 2013. He is working with Dr. Denys Poshyvanyk and his research interests include supporting software development and maintenance tasks for mobile platforms, with a focus on mobile bug and crash reporting. Kevin received his B.S. in Physics with a Minor in Computer Science from the College of the Holy Cross in Worcester, MA in the Spring of 2013. While at Holy Cross Kevin conducted research in atomic physics advised by Dr. Timothy Roach and competed as a varsity athlete in the EARC Collegiate Division 1 rowing league for four years, earning a bid to the IRA national championship regatta in Spring 2013.
